Learning to Demodulate from Few Pilots via Offline and Online Meta-Learning

This paper considers an Internet-of-Things (IoT) scenario in which devices sporadically transmit short packets with few pilot symbols over a fading channel. Devices are characterized by unique transmission non-idealities, such as I/Q imbalance. The number of pilots is generally insufficient to obtain an accurate estimate of the end-to-end channel, which includes the effects of fading and of the transmission-side distortion. This paper proposes to tackle this problem by using meta-learning. Accordingly, pilots from previous IoT transmissions are used as meta-training data in order to train a demodulator that is able to quickly adapt to new end-to-end channel conditions from few pilots. Various state-of-the-art meta-learning schemes are adapted to the problem at hand and evaluated, including Model-Agnostic Meta-Learning (MAML), First-Order MAML (FOMAML), REPTILE, and fast Context Adaptation VIA meta-learning (CAVIA). Both offline and online solutions are developed. In the latter case, an integrated online meta-learning and adaptive pilot number selection scheme is proposed. Numerical results validate the advantages of meta-learning as compared to training schemes that either do not leverage prior transmissions or apply a standard joint learning algorithms on previously received data.

==> remark.tex <==

\newpage
\subsection{Remark}
For general supervised learning problem, under mild conditions, one can consider the learning problem as maximum likelihood problem as
\begin{align} \label{eq:marginal-ml}
\max_\theta p(\mathcal{D}|\theta) = p(s^{(1)}, \ldots, s^{(N)}|y^{(1)},\ldots,y^{(N)},\theta),
\end{align}
where $\mathcal{D} = \{ (s^{(n)},y^{(n)}): n=1,\ldots,N\}$ is a training set containing $N$ training points. More precisely, $s^{(n)}$ is $n$-th \textit{dependent variable, label, response,} or in our communication scenario, transmitted symbol, while $y^{(n)}$ is $n$-th \textit{covariate, domain point, explanatory variable} or in our scenario, received signal \cite{simeone2018brief}. Assuming that we are not interested in \textit{generative probabilistic model}, we can always consider $p(\mathcal{D}|\theta)$ as defined in \eqref{eq:marginal-ml}. All the expressions in this section with $p(\mathcal{D}|\theta)$ is defined as \eqref{eq:marginal-ml} since we are only interested in \textit{discriminative probabilistic model} here.

Now, unlike with general supervised learning problem where inference takes place without any adaptation steps, consider a special learning problem where there exists a dataset which helps inference with adaptation of the parameter $\theta$. This assumption coincides with our scenario where there exists pilot symbols for the meta-test device beforehand of the actual inference. In this case, this adaptation-wise inference can be thought of as introducing a latent variable $\varphi$ with which the inference can actually takes place as,
\begin{align} \label{eq:intro-latent}
p(\mathcal{D}|\theta) = \sum_\varphi p(\varphi|\theta)p(\mathcal{D}|\varphi,\theta).
\end{align}
We can consider this as a \textit{mixture} model where $\varphi$ can be considered as extracted features from dataset $\mathcal{D}$, which in our scenario, can be interpreted as characteristics of current end-to-end channel such as communication channel gain or amplifier's non-linearity.
Now our goal is to find a parameter $\theta$ such that maximizes \eqref{eq:intro-latent}. Since the summation over the latent variables $\varphi$ in \eqref{eq:intro-latent} is complicated, we adopt expectation-maximization (EM) algorithm which finds maximum likelihood estimate of $\theta$ with iterative method \cite{dempster1977maximum, simeone2018brief} guaranteeing convergence to a stationary point of \eqref{eq:intro-latent}. A brief description of EM algorithm is as follows. 

\begin{algorithm}[h] %!
\DontPrintSemicolon
\LinesNumbered
\smallskip
\KwIn{Training set $\mathcal{D} = \{\mathcal{D}_k\}_{k=1,\ldots,K}$}
\smallskip
\KwOut{Learned parameter vector $\theta^{\text{new}}$}
\vspace{0.15cm}
\hrule
\vspace{0.15cm}
{\bf initialize} updated parameter vector $\theta^{\text{old}}$ \\
\texttt{E step}
\smallskip
\begin{align} \label{E-step}
q^{\text{new}}(\varphi) = p(\varphi|\mathcal{D},\theta^{\text{old}}). 
\end{align} \\
\texttt{M step} 
\smallskip
\begin{align} \label{M-step}
\max_\theta Q(\theta,\theta^{\text{old}}) = \mathbb{E}_{\varphi \sim p(\varphi|\mathcal{D},\theta^{\text{old}})}[\log p(\mathcal{D},\varphi|\theta)].
\end{align}
\smallskip \\
If a convergence criterion is not satisfied, set $\theta^{\text{old}} \leftarrow \theta^{\text{new}}$ and return to the E step.
\caption{EM algorithm}
\label{alg:meta-demodulator}
\end{algorithm}

Here, the most tricky part lies in \eqref{E-step}. What is $p(\varphi|\mathcal{D},\theta)?$ However, reminding that we are dealing with discriminative probabilistic model, we can describe $p(\varphi|\mathcal{D},\theta)$ as
\begin{align} \label{latent-dist}
q^{\text{new}}(\varphi) &=  p(\varphi|\mathcal{D},\theta) \\ \label{latent-dist-1}
& = \frac{p(\varphi,\mathcal{D}|\theta)}{p(\mathcal{D}|\theta)} \\ \label{latent-dist-2}
& = \frac{p(\mathcal{D}|\varphi,\theta)p(\varphi|\theta)}{\sum_i p(\mathcal{D},\varphi_i|\theta)} \\ \label{latent-dist-3}
& = \frac{p(\mathcal{D}|\varphi,\theta)p(\varphi|\theta)}{\sum_i [p(\mathcal{D}|\varphi_i,\theta)p(\varphi_i|\theta))]} \\ \label{latent-dist-4}
& = \frac{p(\mathcal{D}_1|\varphi,\theta) \ldots p(\mathcal{D}_K|\varphi,\theta)p(\varphi|\theta) }{\sum_i [p(\mathcal{D}_1|\varphi_i,\theta) \ldots p(\mathcal{D}_K|\varphi_i,\theta)p(\varphi_i|\theta))]} \\ \label{latent-dist-5}
& = \frac{1}{K}(\delta(\varphi=\varphi'_1)+\ldots +\delta(\varphi=\varphi'_K)),
\end{align}
where $\varphi'_k = \xi(\mathcal{D}_k, \theta)$, for $k=1,\ldots,K$ while $\xi: \mathbb{D} \times \Theta \rightarrow \varphi$ is a deterministic function which will be described soon. Here, $\mathbb{D}$ is a space where data points lie in, $\Theta$ is a parameter space for $\theta$, and $\varphi$ is a latent parameter space for $\varphi$. Basically, $\varphi \supseteq \Theta$ but for the special case of MAML, $\varphi =\Theta$, while $\varphi \supset \Theta$ stays for CAVIA. Note that $\varphi'_k$ is a function of $\theta$. Equation \eqref{latent-dist-1} - \eqref{latent-dist-4} comes from basic properties of probability theory along with mutual independence assumption among $\mathcal{D}_1, \ldots, \mathcal{D}_K$. Equation \eqref{latent-dist-5} is not trivial part. Before digging into \eqref{latent-dist-5}, first, let's assume that
\begin{align} \label{laten-dist-5-pf}
p(\mathcal{D}_k|\varphi,\theta) =  \begin{cases} 
\epsilon, \text{  for } \varphi \neq \varphi'_k, \\
\mu, \text{  for } \varphi = \varphi'_k ,
\end{cases}
\end{align}
where $\epsilon << 1$ and $\mu \approx 1$ while $\varphi'_k$ is a proper extracted feature, in other words, proper latent variable, for $\mathcal{D}_k$ given $\theta$. This assumption is nothing but the approximation of  \eqref{eq:marginal-ml} as 
\begin{align} \label{eq:marginal-ml-2}
\nonumber
p(\mathcal{D}_k|\varphi,\theta) &= p(s^{(1)}, \ldots, s^{(N)}|y^{(1)},\ldots,y^{(N)},\varphi,\theta) \\ &\approx \begin{cases} 0, \text{  if latent variable } \varphi \text{ is feature not related with desired class,} \\ 1, \text{  if latent variable } \varphi \text{ is desired class's feature.} \end{cases}
\end{align}
This approximation is straightforward since we are very unlikely to have likelihood of classes that current feature does not stands for. More precisely, if we find $\varphi'_k$ such that maximizes $p(\mathcal{D}_k|\varphi,\theta)$, we can assume \eqref{laten-dist-5-pf} (A more precise way of this illustration is to have local neighborhood of $\varphi'_k$ to have certain probability measure, but here we are assuming that $\varphi'_k$ has a concentrated point probability measure gathered from local neighborhoods). Any function $\xi(\cdot, \cdot)$ that satisfies \eqref{eq:marginal-ml-2} can be used for \eqref{latent-dist-5}. One possible way is to define $\xi(\cdot, \cdot)$ as 
\begin{align} \label{xi-maml}
\xi(\mathcal{D}_k, \theta) = \varphi'_k = \theta + \eta \nabla_\theta \log p(\mathcal{D}_k|\theta).
\end{align}
We can easily check that $\varphi'_k$ from \eqref{xi-maml} maximizes $p(\mathcal{D}_k|\varphi,\theta)$. If \eqref{xi-maml} is insufficient for maximizing $p(\mathcal{D}_k|\varphi,\theta)$, we can take additional gradient steps (multi-step MAML) or any other variant methods.
Now \eqref{latent-dist-1} can then be rewritten as 
\begin{align} \label{latent-dist-4-1}
q^{\text{new}}(\varphi) &= \frac{p(\mathcal{D}_1|\varphi,\theta) \ldots p(\mathcal{D}_K|\varphi,\theta)p(\varphi|\theta) }{\sum_i [p(\mathcal{D}_1|\varphi_i,\theta) \ldots p(\mathcal{D}_K|\varphi_i,\theta)p(\varphi_i|\theta))]}
\\ & \approx 
\frac{p(\mathcal{D}_1|\varphi,\theta) \ldots p(\mathcal{D}_K|\varphi,\theta)p(\varphi|\theta)}{\sum_k \mu \epsilon^{K-1} p(\varphi'_k|\theta)} \\
& \approx
\frac{p(\mathcal{D}_1|\varphi,\theta) \ldots p(\mathcal{D}_K|\varphi,\theta)}{K\mu \epsilon^{K-1}} \\
&=
\begin{cases}
\frac{\mu\epsilon^{K-1}}{K\mu\epsilon^{K-1}} \approx \frac{1}{K} \text{  if  } \varphi \in \{\varphi'_1, \ldots, \varphi'_K\}, \\ 
\frac{\epsilon^{K}}{K\mu\epsilon^{K-1}} \approx 0 \text{  if  } \varphi \not\in \{\varphi'_1, \ldots, \varphi'_K\},
\end{cases}
\end{align}
where we used the property of $\epsilon << 1$, $p(\varphi|\theta)=d\mu$ which does not depend on $\theta$ or $\varphi$ and finally, $q^{\text{new}}(\varphi)$ of being probability measure as \eqref{latent-dist-5}. Now, as we have done with \eqref{E-step}, E step of EM algorithm, the remaining part is M-step, \eqref{M-step}, which is quite straightforward. With \eqref{latent-dist-5}, we can rewrite M step in \eqref{M-step} as,
\begin{align} \label{M-step-final}
\max_\theta \mathbb{E}_{\varphi\sim q^{\text{new}}(\varphi)} [\log p(\mathcal{D},\varphi|\theta)] &= \sum_k \frac{1}{K} \log p(\mathcal{D},\varphi'_k|\theta) \\ &= 
\frac{1}{K}  \sum_k [\log p(\mathcal{D}|\varphi'_k,\theta) + \log p(\varphi'_k|\theta)] \\ &\approx
(K-1)\log \epsilon + \frac{1}{K}\sum_k[ \log p(\mathcal{D}_k|\varphi'_k,\theta) + \log p(\varphi'_k|\theta)] ,
\end{align}
where maximizing 
\begin{align} \label{em-maml-1}
\frac{1}{K}  \sum_k \log p(\mathcal{D}_k|\varphi'_k,\theta) 
\end{align}
is what MAML, Reptile, and CAVIA is actually doing while maximizing \begin{align} \label{em-maml-2}
\frac{1}{K}  \sum_k \log p(\varphi'_k|\theta) 
\end{align}
has not been encountered for previous schemes which can be meaningful to be jointly maximized with \eqref{em-maml-1} in the sense of clustering similar features from different classes to learn common things which have similar features (similar channels, non-linearities, shape, $\ldots$). To write \eqref{em-maml-1} in a more MAML-like way, with \eqref{xi-maml}, we can get
\begin{align} \label{em-maml-final}
\max_\theta \sum_k \log p(\mathcal{D}_k|\varphi'_k,\theta) &= 
\sum_k \log p(\mathcal{D}_k|\theta + \eta \nabla_\theta \log p(\mathcal{D}_k|\theta))
\end{align}
which can be achieved with gradient descent with high order gradients as
\begin{align} \label{em-maml-final2}
\theta \leftarrow \theta + \kappa \nabla_\theta \sum_k  \log p(\mathcal{D}_k|\theta + \eta \nabla_\theta \log p(\mathcal{D}_k|\theta)),
\end{align}
which is exactly same with MAML algorithm.
\newpage























\iffalse
\\
Expectation-maximization (EM) algorithm is an iterative method to find maximum likelihood estimates of parameters given observations which depends on unobserved latent variables \cite{dempster1977maximum}. The way the algorithm finds maximum likelihood estimate, iterating algorithm consisted of expectation step followed by a maximization step, is why it is called EM algorithm. More precisely, suppose observed data $\mathcal{D} = \{\mathcal{D}_k \}_{k=1,\ldots,K}$ follows probability density $p(\mathcal{D}|\varphi;\theta)$ while latent variable $\varphi$ follows probability density $p(\varphi|\theta)$ where $\theta$ is a trainable parameter vector. The goal of EM algorithm is to find $\theta$ that maximizes 
\begin{align} \label{eq:em-goal}
p(\mathcal{D}|\theta) = \int p(\mathcal{D}|\varphi)p(\varphi|\theta)d\varphi,
\end{align}
where $p(\mathcal{D}|\theta)$ is marginal likelihood of the observed data $\mathcal{D}$.
The two steps in each iteration of EM algorithm: expectation step (E-step) and maximization step (M-step) can be expressed as
\begin{align} \label{eq:em-alg}
&\textit{E-step}: Q(\theta|\theta^{(t)}) =  \mathbb{E}_{\varphi|\mathcal{D},\theta^{(t)}}[\log p(\mathcal{D|\varphi}) + \log p(\varphi|\theta)] \\
&\textit{M-step}:
\theta^{(t+1)} = \argmax_\theta Q(\theta|\theta^{(t)})
\end{align}
where $\theta^{(t)}$ is estimate of parameter $\theta$ at $t$-th iteration.

Now, we will show that general probabilistic model for meta-learning can be seen as approximation of EM algorithm. First of all, we redefine EM algorithm as 
\begin{align} \label{eq:em-alg-ours}
&\textit{E-step}: Q(\theta) =  \mathbb{E}_{\varphi|\mathcal{D},\theta}[\log p(\mathcal{D|\varphi}) + \log p(\varphi|\theta)] \\
&\textit{M-step}:
\theta \leftarrow \theta + \kappa \nabla_\theta Q(\theta),
\end{align}
where $\varphi = \varphi(\theta)$ which keeps dependency of $\theta$ for gradient calculation. This slight change of the algorithm lets the algorithm only to look local neighborhood of $\theta$ which lies as basic assumption of deep learning. (cite? deep learning? sgd? gd? ...)

\begin{align} \label{eq:e-part-1}
Q(\theta) =  \mathbb{E}_{\varphi|\mathcal{D},\theta}\left[\sum_i \log p(\mathcal{D}_i|\varphi) + \log p(\varphi|\theta)\right],
\end{align}
since we are assuming data points $\mathcal{D}_i, i=1,\ldots,K$ are independent. Now let's get the approximation of the conditional distribution $p(\varphi|\mathcal{D},\theta)$ as
\begin{align} \label{eq:e-part-2}
p(\varphi|\mathcal{D},\theta) = \begin{cases} \varphi'_1 \text{  with probability } \frac{1}{K} \\ \varphi'_2 \text{  with probability } \frac{1}{K}\\ \vdots \\ \varphi'_K \text{  with probability }\frac{1}{K}, \end{cases}
\end{align}
which follows naturally from the point estimate of (\textit{Appendix A}?? how to cite....)
\begin{align} \label{eq:e-part-3}
p(\varphi|\mathcal{D}_k,\theta) \approx \delta(\varphi = \varphi'_k).
\end{align}
Now, \eqref{eq:e-part-1} becomes 
\begin{align} \label{eq:e-part-4}
Q(\theta) &\approx \sum_k \frac{1}{K} \left[\sum_i \log p(\mathcal{D}_i|\varphi'_k) + \log p(\varphi'_k|\theta)\right]
\end{align}
\begin{align} \label{eq:e-part-5}
\nabla_\theta Q(\theta) = \sum_k \frac{1}{K} \nabla_\theta \log p(\mathcal{D}_i|\varphi'_k)
\end{align}

$\sum_{i\neq k}p(\mathcal{D}_i|\varphi'_k) = const.$ from the assumption \eqref{eq:e-part-3}. 
If $\varphi \in \Theta $, then MAML, if $\varphi \in \Theta \cup \mathcal{C}$, then CAVIA. How to update $\theta$ given $\varphi \in \Theta $, variations such as FOMAML and REPTILE comes.
\fi



